The spectroscopic binary fraction of the young stellar cluster M17

Significant progress has been made toward understanding the formation of massive ($M > 8~$M$_{\odot}$) binaries in close orbits. For example, the detection of a very low velocity dispersion among the massive stars in the young region M17 and the measurement of a positive trend of velocity dispersion with age in Galactic clusters. The velocity dispersion observed in M17 could be explained either by the lack of binaries among the stars in this region or by larger binary separations than typically observed, but with a binary fraction similar to other young Galactic clusters. The latter implies that over time, the binary components migrate toward each other. We aim to determine the origin of the strikingly low velocity dispersion by determining the observed and intrinsic binary fraction of massive stars in M17 through multi-epoch spectroscopy. We performed a multi-epoch spectroscopic survey consisting of three epochs separated by days and months. We determine the radial velocity of each star at each epoch by fitting the stellar absorption profiles. We determine an observed binary fraction of 27% and an intrinsic binary fraction of 87%, consistent with that of other Galactic clusters. We conclude that the low velocity dispersion is due to a large separation among the young massive binaries in M17. Our result is in agreement with a migration scenario in which massive stars are born in binaries or higher order systems at large separation and harden within the first million years of evolution. Such an inward migration may either be driven by interaction with a remnant accretion disk, with other young stellar objects present in the system or by dynamical interactions within the cluster. Our results imply that possibly both dynamical interactions and binary evolution are key processes in the formation of gravitational wave sources.

==> overview_table.tex <==
\onecolumn
\begin{longtable}{ccccccccc}
\caption{\label{kstars} Sample stars with absolute magnitude}\\
\hline\hline
& starname &        date & $v_{Gwc}$ (km/s) & $v_{Gnc}$ (km/s) & $v_{Lwc}$ (km/s) & $v_{Lnc}$ (km/s) & $v_{Vwc}$ (km/s) & $v_{Vnc}$ (km/s) \\
\hline
    1 & B86 & 20190706T01 &        $3 \pm 2$ &   $-3.7 \pm 0.3$ &        $3 \pm 3$ &   $-3.8 \pm 0.4$ &        $4 \pm 2$ &   $ -4 \pm NaN $ \\
    &  & 20190709T00 &      $-26 \pm 2$ &  $-30.8 \pm 0.3$ &      $-26 \pm 3$ &  $-34.5 \pm 0.3$ &      $-26 \pm 2$ &  $ -32 \pm NaN $ \\
    &  & 20190803T03 &      $-26 \pm 2$ &  $-33.7 \pm 0.2$ &      $-26 \pm 3$ &  $-32.4 \pm 0.2$ &      $-26 \pm 2$ &  $ -35 \pm NaN $ \\
    \hline
    2 & B253 & 20190605T06 &       $-5 \pm 2$ &      $-15 \pm 3$ &       $-4 \pm 2$ &       $-8 \pm 3$ &   $ -5 \pm NaN $ &  $ -12 \pm NaN $ \\
    & & 20190607T06 &       $-3 \pm 2$ &      $-11 \pm 3$ &       $-5 \pm 2$ &       $-8 \pm 4$ &   $ -6 \pm NaN $ &  $ -10 \pm NaN $ \\
    & & 20190709T02 &       $26 \pm 2$ &       $24 \pm 3$ &       $22 \pm 2$ &       $15 \pm 3$ &   $ 24 \pm NaN $ &   $ 22 \pm NaN $ \\
    \hline
    3 & B230 & 20190730T04 &     $-20 \pm 10$ &     $-10 \pm 10$ &       $-9 \pm 9$ &       $0 \pm 10$ &       $0 \pm 10$ &   $ -0 \pm NaN $ \\
    & & 20190801T02 &     $-10 \pm 10$ &      $10 \pm 10$ &      $-19 \pm 9$ &        $4 \pm 9$ &       $10 \pm 9$ &    $ 4 \pm NaN $ \\
    & & 20190829T00 &       $0 \pm 10$ &      $20 \pm 10$ &        $4 \pm 9$ &      $10 \pm 10$ &       $0 \pm 10$ &   $ 10 \pm NaN $ \\
    \hline
    4 & B290 & 20190706T01 &       $14 \pm 3$ &   $22.3 \pm 0.6$ &       $10 \pm 3$ &   $13.0 \pm 0.6$ &   $ 11 \pm NaN $ &   $ 13 \pm NaN $ \\
    & & 20190709T00 &       $12 \pm 3$ &   $19.6 \pm 0.6$ &        $8 \pm 3$ &   $11.5 \pm 0.7$ &   $ 10 \pm NaN $ &   $ 11 \pm NaN $ \\
    & & 20190809T00 &        $5 \pm 3$ &   $12.7 \pm 0.7$ &        $2 \pm 3$ &    $3.9 \pm 0.7$ &    $ 3 \pm NaN $ &    $ 4 \pm NaN $ \\
    \hline
    5 & B311 & 20190501T08 &        $7 \pm 1$ &       $13 \pm 4$ &        $8 \pm 1$ &       $23 \pm 3$ &        $8 \pm 1$ &   $ 22 \pm NaN $ \\
    & & 20190502T09 &        $1 \pm 1$ &       $18 \pm 4$ &        $4 \pm 1$ &       $19 \pm 4$ &        $3 \pm 1$ &   $ 19 \pm NaN $ \\
    & & 20190605T07 &        $7 \pm 1$ &       $21 \pm 6$ &        $9 \pm 1$ &      $20 \pm 20$ &        $9 \pm 1$ &   $ 23 \pm NaN $ \\
    \hline
    6 & B164 & 20190605T06 &        $7 \pm 3$ &        $7 \pm 2$ &       $10 \pm 2$ &        $8 \pm 2$ &    $ 8 \pm NaN $ &    $ 6 \pm NaN $ \\
    & & 20190607T06 &       $10 \pm 3$ &        $9 \pm 3$ &       $11 \pm 2$ &        $8 \pm 2$ &   $ 11 \pm NaN $ &    $ 9 \pm NaN $ \\
    & & 20190710T00 &        $5 \pm 3$ &        $8 \pm 2$ &        $7 \pm 2$ &        $6 \pm 2$ &    $ 6 \pm NaN $ &    $ 6 \pm NaN $ \\
    \hline
    7 & B215 & 20190730T05 &       $19 \pm 5$ &       $16 \pm 3$ &       $13 \pm 4$ &       $10 \pm 4$ &   $ 14 \pm NaN $ &   $ 11 \pm NaN $ \\
    & & 20190804T03 &       $12 \pm 5$ &        $8 \pm 2$ &        $8 \pm 4$ &        $7 \pm 2$ &    $ 8 \pm NaN $ &    $ 4 \pm NaN $ \\
    & & 20190927T23 &        $9 \pm 5$ &        $5 \pm 2$ &        $7 \pm 4$ &        $5 \pm 3$ &    $ 8 \pm NaN $ &    $ 4 \pm NaN $ \\
    \hline
    8 & B268 & 20190530T08 &       $13 \pm 6$ &   $13.1 \pm 0.5$ &       $12 \pm 5$ &   $11.4 \pm 0.8$ &       $13 \pm 5$ &   $ 14 \pm NaN $ \\
    & & 20190531T07 &       $13 \pm 6$ &        $8 \pm 1$ &        $6 \pm 5$ &    $3.3 \pm 0.9$ &       $11 \pm 5$ &    $ 2 \pm NaN $ \\
    & & 20190729T04 &        $6 \pm 6$ &      $-12 \pm 1$ &       $-3 \pm 5$ &      $-23 \pm 1$ &        $4 \pm 5$ &  $ -16 \pm NaN $ \\
    \hline
    9 & B205 & 20190605T05 &       $14 \pm 4$ &        $7 \pm 1$ &       $16 \pm 4$ &       $10 \pm 2$ &   $ 17 \pm NaN $ &    $ 7 \pm NaN $ \\
    & & 20190606T05 &       $41 \pm 4$ &       $40 \pm 4$ &       $46 \pm 4$ &       $52 \pm 5$ &   $ 45 \pm NaN $ &   $ 56 \pm NaN $ \\
    & & 20190706T05 &       $30 \pm 4$ &       $34 \pm 1$ &       $25 \pm 4$ &       $25 \pm 2$ &   $ 26 \pm NaN $ &   $ 32 \pm NaN $ \\
    \hline
    10 & B111 & 20190411T09 &        $2 \pm 1$ &       $-3 \pm 1$ &        $4 \pm 2$ &        $2 \pm 2$ &    $ 4 \pm NaN $ &   $ -1 \pm NaN $ \\
    & & 20190413T08 &        $1 \pm 1$ &       $-1 \pm 1$ &        $3 \pm 1$ &        $2 \pm 2$ &    $ 3 \pm NaN $ &    $ 1 \pm NaN $ \\
    & & 20190605T05 &       $-3 \pm 1$ &       $-7 \pm 2$ &       $-1 \pm 1$ &       $-3 \pm 2$ &   $ -1 \pm NaN $ &   $ -5 \pm NaN $ \\
    \hline
    11 & B336 & 20190706T04 &       $28 \pm 4$ &   $ 27 \pm NaN $ &       $25 \pm 4$ &   $ 24 \pm NaN $ &       $25 \pm 4$ &   $ 26 \pm NaN $ \\
    & & 20190709T01 &       $48 \pm 4$ &   $ 48 \pm NaN $ &       $45 \pm 4$ &   $ 45 \pm NaN $ &       $45 \pm 4$ &   $ 45 \pm NaN $ \\
    & & 20190809T01 &       $52 \pm 4$ &   $ 52 \pm NaN $ &       $50 \pm 4$ &   $ 50 \pm NaN $ &       $50 \pm 4$ &   $ 50 \pm NaN $ \\
    \hline
    12 & B150 & 20190706T04 &       $29 \pm 3$ &       $27 \pm 3$ &       $22 \pm 3$ &       $16 \pm 4$ &   $ 25 \pm NaN $ &   $ 26 \pm NaN $ \\
    & & 20190709T01 &       $37 \pm 3$ &       $27 \pm 4$ &       $32 \pm 3$ &       $27 \pm 4$ &   $ 34 \pm NaN $ &   $ 23 \pm NaN $ \\
    & & 20190809T00 &        $9 \pm 3$ &        $2 \pm 3$ &       $12 \pm 3$ &        $6 \pm 4$ &   $ 11 \pm NaN $ &    $ 4 \pm NaN $ \\
    \hline
    13 & 326 & 20190706T01 &      $-14 \pm 4$ &      $-17 \pm 2$ &      $-20 \pm 4$ &      $-25 \pm 3$ &      $-17 \pm 4$ &  $ -19 \pm NaN $ \\
    &  & 20190709T00 &       $10 \pm 4$ &      $-10 \pm 2$ &        $8 \pm 4$ &       $-7 \pm 3$ &        $9 \pm 4$ &   $ -7 \pm NaN $ \\
    &  & 20190809T00 &       $41 \pm 4$ &       $38 \pm 2$ &       $54 \pm 4$ &       $53 \pm 2$ &       $46 \pm 4$ &   $ 53 \pm NaN $ \\
    \hline
    14 & B243 & 20190730T03 &     $-20 \pm 10$ &      $-20 \pm 3$ &      $-26 \pm 9$ &      $-24 \pm 2$ &      $-26 \pm 9$ &  $ -19 \pm NaN $ \\
    & & 20190803T04 &      $20 \pm 10$ &       $23 \pm 3$ &       $23 \pm 9$ &       $38 \pm 3$ &       $32 \pm 9$ &   $ 34 \pm NaN $ \\
    & & 20190925T01 &       $0 \pm 10$ &        $2 \pm 3$ &       $-8 \pm 9$ &      $-11 \pm 2$ &       $0 \pm 10$ &   $ -9 \pm NaN $ \\
    \hline
    15 & B275 & 20190605T07 &       $23 \pm 2$ &       $18 \pm 5$ &       $18 \pm 2$ &       $12 \pm 6$ &       $21 \pm 2$ &   $ 14 \pm NaN $ \\
    & & 20190606T05 &       $12 \pm 2$ &      $20 \pm 10$ &       $11 \pm 2$ &       $13 \pm 9$ &       $12 \pm 2$ &   $ 16 \pm NaN $ \\
    & & 20190709T02 &       $25 \pm 2$ &       $21 \pm 6$ &       $18 \pm 2$ &       $15 \pm 7$ &       $23 \pm 2$ &   $ 19 \pm NaN $ \\
    \hline
    16 & B93 & 20190624T06 &        $8 \pm 2$ &   $14.9 \pm 0.2$ &        $6 \pm 3$ &   $11.4 \pm 0.5$ &        $6 \pm 3$ &   $ 11 \pm NaN $ \\
    &  & 20190808T23 &        $7 \pm 2$ &   $12.6 \pm 0.2$ &        $6 \pm 3$ &   $11.4 \pm 0.4$ &        $6 \pm 3$ &   $ 11 \pm NaN $ \\
    \hline
    17 & B269 & 20190614T05 &      $10 \pm 10$ &        $7 \pm 5$ &      $10 \pm 10$ &       $12 \pm 3$ &   $ 11 \pm NaN $ &   $ 12 \pm NaN $ \\
    & & 20190712T02 &       $0 \pm 10$ &       $0 \pm 20$ &      $10 \pm 10$ &      $30 \pm 80$ &    $ 9 \pm NaN $ &    $ 1 \pm NaN $ \\
    \hline
    18 & B289 & 20190518T09 &       $-9 \pm 5$ &      $-10 \pm 4$ &       $-7 \pm 4$ &       $-5 \pm 2$ &   $ -8 \pm NaN $ &   $ -5 \pm NaN $ \\
    & & 20190624T04 &        $2 \pm 5$ &        $9 \pm 5$ &        $3 \pm 4$ &        $2 \pm 3$ &    $ 3 \pm NaN $ &    $ 2 \pm NaN $ \\ 
    \hline
    19 & B337 & 20190501T07 &       $-2 \pm 4$ &   $ -1 \pm NaN $ &        $0 \pm 3$ &    $ 0 \pm NaN $ &        $0 \pm 3$ &    $ 0 \pm NaN $ \\
    & & 20190803T01 &       $-4 \pm 4$ &   $ -7 \pm NaN $ &       $-6 \pm 3$ &   $ -7 \pm NaN $ &       $-6 \pm 5$ &   $ -7 \pm NaN $ \\
    \hline
    20 & B272 & 20190805T01 &        $4 \pm 6$ &       $0 \pm 20$ &        $2 \pm 4$ &       $0 \pm 20$ &    $ 2 \pm NaN $ &    $ 4 \pm NaN $ \\
    \hline
    21 & B213 & 20190804T05 &       $-6 \pm 9$ &       $-4 \pm 8$ &      $-12 \pm 7$ &      $-15 \pm 3$ &      $-14 \pm 8$ &  $ -15 \pm NaN $ \\
    \hline
    22 & B234 & 20190805T02 &     $-10 \pm 10$ &       $0 \pm 10$ &       $-5 \pm 9$ &       $0 \pm 10$ &     $-10 \pm 10$ &       $0 \pm 10$ \\
    \hline
    23 & B181 & 20190804T04 &        $2 \pm 7$ &        $1 \pm 1$ &        $1 \pm 5$ &       $-2 \pm 2$ &    $ 1 \pm NaN $ &   $ -2 \pm NaN $ \\
    \hline
    24 & CEN55 & 20190805T03 &       $12 \pm 3$ &      $10 \pm 10$ &       $13 \pm 3$ &       $13 \pm 8$ &       $13 \pm 3$ &   $ 13 \pm NaN $ \\
\hline
% \end{tabular}
\label{P4:tab:EW_early}
\end{longtable}
\twocolumn
